Semi-Supervised Semantic Segmentation with High- and Low-level Consistency

The ability to understand visual information from limited labeled data is an important aspect of machine learning. While image-level classification has been extensively studied in a semi-supervised setting, dense pixel-level classification with limited data has only drawn attention recently. In this work, we propose an approach for semi-supervised semantic segmentation that learns from limited pixel-wise annotated samples while exploiting additional annotation-free images. It uses two network branches that link semi-supervised classification with semi-supervised segmentation including self-training. The dual-branch approach reduces both the low-level and the high-level artifacts typical when training with few labels. The approach attains significant improvement over existing methods, especially when trained with very few labeled samples. On several standard benchmarks - PASCAL VOC 2012, PASCAL-Context, and Cityscapes - the approach achieves new state-of-the-art in semi-supervised learning.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> egbib.tex <==

%%--------------------fully-supervised semantic segmentation ---------------------------------------------


@article{DBLP:journals/corr/ChenPKMY14,
  author    = {Liang{-}Chieh Chen and
               George Papandreou and
               Iasonas Kokkinos and
               Kevin Murphy and
               Alan L. Yuille},
  title     = {Semantic Image Segmentation with Deep Convolutional Nets and Fully
               Connected CRFs},
  journal   = {CoRR},
  volume    = {abs/1412.7062},
  year      = {2014},
}

@InProceedings{Zhang_2018_CVPR,
author = {Zhang, Hang and Dana, Kristin and Shi, Jianping and Zhang, Zhongyue and Wang, Xiaogang and Tyagi, Ambrish and Agrawal, Amit},
title = {Context Encoding for Semantic Segmentation},
booktitle = {CVPR},
year = {2018}
}

@InProceedings{Chen_2018_ECCV,
author= {Liang{-}Chieh Chen and Yukun Zhu and George Papandreou and Florian Schroff and Hartwig Adam},
title={Encoder-Decoder with Atrous Separable Convolution for Semantic Image Segmentation},
booktitle={ECCV},
year={2018},
}

@article{DBLP:journals/pami/ChenPKMY18,
  author    = {Liang{-}Chieh Chen and George Papandreou and Iasonas Kokkinos and Kevin Murphy and Alan L. Yuille},
  title     = {DeepLab: Semantic Image Segmentation with Deep Convolutional Nets, Atrous Convolution, and Fully Connected CRFs},
  journal   = {TPAMI},
  volume    = {40},
  number    = {4},
  pages     = {834--848},
  year      = {2018},
  }
  
  
@InProceedings{Peng_2017_CVPR,
author = {Peng, Chao and Zhang, Xiangyu and Yu, Gang and Luo, Guiming and Sun, Jian},
title = {Large Kernel Matters -- Improve Semantic Segmentation by Global Convolutional Network},
booktitle = {CVPR},
year = {2017}
}

@InProceedings{Lin_2017_CVPR,
author = {Lin, Guosheng and Milan, Anton and Shen, Chunhua and Reid, Ian},
title = {RefineNet: Multi-Path Refinement Networks for High-Resolution Semantic Segmentation},
booktitle = {CVPR},
year = {2017}
}

@InProceedings{Long_2015_CVPR,
author = {Long, Jonathan and Shelhamer, Evan and Darrell, Trevor},
title = {Fully Convolutional Networks for Semantic Segmentation},
booktitle = {CVPR},
year = {2015},
}


%% -------------------weakly-supervised semantic segmentation ---------------------------------------------
@InProceedings{Lin_2016_CVPR,
author = {Lin, Di and Dai, Jifeng and Jia, Jiaya and He, Kaiming and Sun, Jian},
title = {ScribbleSup: Scribble-Supervised Convolutional Networks for Semantic Segmentation},
booktitle = {CVPR},
year = {2016}
}

@InProceedings{Dai_2015_ICCV,
author = {Dai, Jifeng and He, Kaiming and Sun, Jian},
title = {BoxSup: Exploiting Bounding Boxes to Supervise Convolutional Networks for Semantic Segmentation},
booktitle = {ICCV},
year = {2015}
}

@InProceedings{Ahn_2018_CVPR,
author = {Ahn, Jiwoon and Kwak, Suha},
title = {Learning Pixel-Level Semantic Affinity With Image-Level Supervision for Weakly Supervised Semantic Segmentation},
booktitle = {CVPR},
year = {2018}
}

@InProceedings{Pinheiro_2015_CVPR,
author = {Pinheiro, Pedro O. and Collobert, Ronan},
title = {From Image-Level to Pixel-Level Labeling With Convolutional Networks},
booktitle = {CVPR},
year = {2015}
}

@InProceedings{Meng_2018_ECCV,
author= {Tang, Meng and Perazzi, Federico and Djelouah, Abdelaziz and Ayed, Ismail Ben and Schroers, Christopher and Boykov, Yuri},
title={On Regularized Losses for Weakly-supervised CNN Segmentation},
booktitle={ECCV},
year={2018},
}

@InProceedings{Ahn_2018_CVPR,
author = {Ahn, Jiwoon and Kwak, Suha},
title = {Learning Pixel-Level Semantic Affinity With Image-Level Supervision for Weakly Supervised Semantic Segmentation},
booktitle = {CVPR},
year = {2018}
}

@InProceedings{Wei_2017_CVPR,
author = {Wei, Yunchao and Feng, Jiashi and Liang, Xiaodan and Cheng, Ming-Ming and Zhao, Yao and Yan, Shuicheng},
title = {Object Region Mining With Adversarial Erasing: A Simple Classification to Semantic Segmentation Approach},
booktitle = {CVPR},
year = {2017}
}

%%------------------- semi-supervised approaches with extra weak annotations--------------------------------

@InProceedings{Wei_2018_CVPR,
author = {Wei, Yunchao and Xiao, Huaxin and Shi, Honghui and Jie, Zequn and Feng, Jiashi and Huang, Thomas S.},
title = {Revisiting Dilated Convolution: A Simple Approach for Weakly- and Semi-Supervised Semantic Segmentation},
booktitle = {CVPR},
year = {2018}
}

@InProceedings{Papandreou_2015_ICCV,
author = {Papandreou, George and Chen, Liang-Chieh and Murphy, Kevin P. and Yuille, Alan L.},
title = {Weakly- and Semi-Supervised Learning of a Deep Convolutional Network for Semantic Image Segmentation},
booktitle = {ICCV},
year = {2015}
}

%% with extra bounding boxes
@InProceedings{Khoreva_2017_CVPR,
author = {Khoreva, Anna and Benenson, Rodrigo and Hosang, Jan and Hein, Matthias and Schiele, Bernt},
title = {Simple Does It: Weakly Supervised Instance and Semantic Segmentation},
booktitle = {CVPR},
year = {2017}
}

%%--------------------------GAN/semi-supervised methods-------------------------------------------

@InProceedings{Hung_2018_BMVC,
author = {Wei{-}Chih Hung and Yi{-}Hsuan Tsai and Yan{-}Ting Liou and Yen{-}Yu Lin and Ming{-}Hsuan Yang},
title = {Adversarial Learning for Semi-Supervised Semantic Segmentation},
booktitle = {BMVC},
year = {2018}
}

@incollection{Luc2016SemanticSU,
  title={Semantic Segmentation using Adversarial Networks},
  author={Pauline Luc and Camille Couprie and Soumith Chintala and Jakob Verbeek},
  booktitle={NIPS Workshops},
  year={2016}
}

@InProceedings{Souly_2017_ICCV,
author = {Souly, Nasim and Spampinato, Concetto and Shah, Mubarak},
title = { Semi Supervised Semantic Segmentation Using Generative Adversarial Network},
booktitle = {ICCV},
year = {2017}
}

@incollection{NIPS2014_5423,
title = {Generative Adversarial Nets},
author = {Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
booktitle = {NIPS},
year = {2014},
}

%% ------------------------ using Classification network ----------------------------------------

@incollection{NIPS2015_5858,
title = {Decoupled Deep Neural Network for Semi-supervised Semantic Segmentation},
author = {Hong, Seunghoon and Noh, Hyeonwoo and Han, Bohyung},
booktitle = {NIPS},
year = {2015}
}

%% -------------------------semi-supervised classification----------------------------------------

@incollection{NIPS2017_6719,
title = {Mean teachers are better role models: Weight-averaged consistency targets improve semi-supervised deep learning results},
author = {Tarvainen, Antti and Valpola, Harri},
booktitle = {NIPS},
year = {2017} 
}

@article{athiwaratkun2018improving,
  title={Improving Consistency-Based Semi-Supervised Learning with Weight Averaging},
  author={Athiwaratkun, Ben and Finzi, Marc and Izmailov, Pavel and Wilson, Andrew Gordon},
  journal={arXiv preprint arXiv:1806.05594},
  year={2018}
}

@incollection{improvedGAN,
title = {Improved Techniques for Training GANs},
author = {Salimans, Tim and Goodfellow, Ian and Zaremba, Wojciech and Cheung, Vicki and Radford, Alec and Chen, Xi and Chen, Xi},
booktitle = {NIPS},
year = {2016},
}

@incollection{
  oliver2018realistic,
  title={Realistic Evaluation of Semi-Supervised Learning Algorithms},
  author={Avital Oliver and Augustus Odena and Colin Raffel and Ekin D. Cubuk and Ian J. Goodfellow},
  booktitle = {ICLR Workshop },
  year={2018}
}

@article{Miyato2018VirtualAT,
  title={Virtual Adversarial Training: a Regularization Method for Supervised and Semi-supervised Learning},
  author={Takeru Miyato and Shin-ichi Maeda and Masanori Koyama and Shin Ishii},
  journal={TPAMI},
  year={2018}
}

@inproceedings{Laine2017, 
  author =    {Samuli Laine and Timo Aila},
  title =     {Temporal Ensembling for Semi-Supervised Learning},
  booktitle =   {ICLR},
  year =      {2017},
}


%% -----------------------------  Datasets---------------------------------------------------------
@InProceedings{Mottaghi_2014_CVPR,
author = {Mottaghi, Roozbeh and Chen, Xianjie and Liu, Xiaobai and Cho, Nam-Gyu and Lee, Seong-Whan and Fidler, Sanja and Urtasun, Raquel and Yuille, Alan},
title = {The Role of Context for Object Detection and Semantic Segmentation in the Wild},
booktitle = {CVPR},
year = {2014}
}

@article{pascal_voc,
 author = {Everingham, Mark and Gool, Luc and Williams, Christopher K. and Winn, John and Zisserman, Andrew},
 title = {The Pascal Visual Object Classes (VOC) Challenge},
 journal = {IJCV},
 issue_date = {2010},
 volume = {88},
 number = {2},
 year = {2010},
 pages = {303--338},
} 

@InProceedings{Cordts_2016_CVPR,
author = {Cordts, Marius and Omran, Mohamed and Ramos, Sebastian and Rehfeld, Timo and Enzweiler, Markus and Benenson, Rodrigo and Franke, Uwe and Roth, Stefan and Schiele, Bernt},
title = {The Cityscapes Dataset for Semantic Urban Scene Understanding},
booktitle = {CVPR},
year = {2016}
}


@INPROCEEDINGS{Deng09imagenet:a,
    author = {Jia Deng and Wei Dong and Richard Socher and Li-jia Li and Kai Li and Li Fei-fei},
    title = {Imagenet: A large-scale hierarchical image database},
    booktitle = {CVPR},
    year = {2009}
}


@inproceedings{mscoco,
    title = {Microsoft {COCO}: Common Objects in Context},
    author = {Tsung-Yi Lin and Michael Maire and Serge Belongie and James Hays and Pietro Perona and Deva Ramanan and Piotr Dollár and C. Lawrence Zitnick},
    booktitle = {ECCV},
    year = {2014},
}

@InProceedings{BharathICCV2011,
author = "Bharath Hariharan and Pablo Arbelaez and Lubomir Bourdev and Subhransu Maji and Jitendra Malik",
title = "Semantic Contours from Inverse Detectors",
booktitle = "ICCV",
year = "2011",
}

%% ------------------------------Libraries & Code-------------------------------------------------------

@article{paszke2017automatic,
  title={Automatic differentiation in PyTorch},
  author={Paszke, Adam and Gross, Sam and Chintala, Soumith and Chanan, Gregory and Yang, Edward and DeVito, Zachary and Lin, Zeming and Desmaison, Alban and Antiga, Luca and Lerer, Adam},
  booktitle={NIPS Workshops},
  year={2017}
}



%% ------------------------------Networks----------------------------------------------------------

@InProceedings{He_2016_CVPR,
author = {He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
title = {Deep Residual Learning for Image Recognition},
booktitle = {CVPR},
year = {2016}
}

@INPROCEEDINGS{Maas13rectifiernonlinearities,
    author = {Andrew L. Maas and Awni Y. Hannun and Andrew Y. Ng},
    title = {Rectifier nonlinearities improve neural network acoustic models},
    booktitle = {ICML Workshop on Deep Learning for Audio, Speech and Language Processing},
    year = {2013}
}

@article{Srivastava:2014:DSW:2627435.2670313,
 author = {Srivastava, Nitish and Hinton, Geoffrey and Krizhevsky, Alex and Sutskever, Ilya and Salakhutdinov, Ruslan},
 title = {Dropout: A Simple Way to Prevent Neural Networks from Overfitting},
 journal = {JMLR},
 volume = {15},
 number = {1},
 year = {2014},
 pages = {1929--1958},
 numpages = {30},
} 

%%-----------------------------------Self-training for SSL-----------------------------------------
@MISC{Zhu06semi-supervisedlearning,
    author = {Xiaojin Zhu},
    title = {Semi-Supervised Learning Literature Survey},
    year = {2006}
}


@book{Chapelle:2010:SL:1841234,
 author = {Chapelle, Olivier and Schlkopf, Bernhard and Zien, Alexander},
 title = {Semi-Supervised Learning},
 year = {2010},
 isbn = {0262514125, 9780262514125},
} 


%%-----------------------------------Miscellaneous/Introduction--------------------------------------------------

@INPROCEEDINGS{Lecun98gradient-basedlearning,
    author = {Yann Lecun and Léon Bottou and Yoshua Bengio and Patrick Haffner},
    title = {Gradient-based learning applied to document recognition},
    booktitle = {Proceedings of the IEEE},
    year = {1998},
    pages = {2278--2324}
}

@incollection{NIPS2017_6639,
title = {Semi-Supervised Learning for Optical Flow with Generative Adversarial Networks},
author = {Lai, Wei-Sheng and Huang, Jia-Bin and Yang, Ming-Hsuan},
booktitle = {NIPS},
year = {2017},
}


@incollection{NIPS2011_4296,
title = {Efficient Inference in Fully Connected CRFs with Gaussian Edge Potentials},
author = {Philipp Kr\"{a}henb\"{u}hl and Koltun, Vladlen},
booktitle = {NIPS},
year = {2011},
}

@inproceedings{hu2018senet,
  title={Squeeze-and-Excitation Networks},
  author={Jie Hu and Li Shen and Gang Sun},
  booktitle={CVPR},
  year={2018},
}


@InProceedings{kingma:adam,
author = {Kingma, Diederick P and Ba, Jimmy},
title = {Adam: A method for stochastic optimization},
booktitle = {ICLR},
year = {2015}
}


